HTN Plan Repair Algorithms Compared: Strengths and Weaknesses of Different Methods

This paper provides theoretical and empirical comparisons of three recent hierarchical plan repair algorithms: SHOPFixer, IPyHOPPER, and Rewrite. Our theoretical results show that the three algorithms correspond to three different definitions of the plan repair problem, leading to differences in the algorithms' search spaces, the repair problems they can solve, and the kinds of repairs they can make. Understanding these distinctions is important when choosing a repair method for any given application. Building on the theoretical results, we evaluate the algorithms empirically in a series of benchmark planning problems. Our empirical results provide more detailed insight into the runtime repair performance of these systems and the coverage of the repair problems solved, based on algorithmic properties such as replanning, chronological backtracking, and backjumping over plan trees.

==> plan-repair.tex <==
\section{Hierarchical Plan Repair Strategies}
\label{sec:plan-repair}

%

\input{qualitative-differences}






We now will briefly summarize the three hierarchical plan
repair algorithms that we have evaluated in this work.

\subsection{\shopfixer{} Plan Repair}
\label{sec:shopfixer-alg}

\shopfixer \cite{GoldmanETAL:PlanRepair:2020} is a method for repairing plans
generated by the forward-searching HTN planner, \shop. It uses
a graph of causal links and task decompositions to identify a minimal
subset of the plan that must be fixed. \shopfixer
extends the notion of plan repair stability introduced by
\cite{fox06plan}, and further develop their methods and experiments,
which showed the advantages of plan repair over replanning.


The basic idea behind \shopfixer's plan repair approach is very
simple: when a disturbance is introduced into the plan, \shopfixer
finds the minimal subtree of the plan tree that contains the node
whose preconditions are clobbered by that disturbance: the failure
node. If there is no such node, then the disturbance does not
interfere with the success of the plan. \shopfixer will then repair
the plan, starting with the minimal subtree. To find the minimal
subtree around a failure node, \shopfixer finds the first task in the
plan that is potentially ``clobbered'' (rendered unexecutable) by that
disturbance, and restarts the planning search from that task's
immediate parent in the HTN plan (since that was where
that task was chosen for insertion into the plan). This plan repair is
done by {\em backjumping} into the search stack for SHOP3 and
reconstructing the compromised subtree without the later tasks. Note
that the first clobbered task may be either a primitive task or a
complex task. Furthermore, if $p$ is the parent of child $c$ in an HTN
plan, then $p$'s preconditions are considered chronologically prior to
$c$'s, because it is the satisfaction of $p$'s preconditions that
enables $c$ to be introduced into the plan: if both $p$ and $c$ fail,
and we repair only $c$, we will still have a failed plan, because
after the disturbance, we are not licensed to insert $c$ or its
successor nodes.


\shopfixer restarts the planning search by backjumping to the
corresponding entry in the SHOP3 search stack, which it retains, and
updating the world state at that point with the effects of the
disturbance. When restarting the planning search, \shopfixer
``freezes'' the prefix of the plan that has already been executed, as
well as the deviation and its effects. It may backjump to decisions
prior to the deviation, for example, if the immediate parent of the
failed task is the top level task of the problem, but it cannot undo
the effects of an action that is already done. \shopfixer returns a
repaired plan that is made up of the prefix before the disturbance,
the disturbance, and the repaired suffix.

\subsection{IPyHOPPER Plan Repair}
\label{sec:ipyhopper-alg}

\ipyhopper{} \cite{Zaidins:HPlan2023} is a progression based HTN planner written in Python.
The primary distinction between \ipyhopper{} and other HTN planning
and plan repair methods is that it does not use projection.  Instead,
it uses an external simulator to predict the effects of planned actions.

\ipyhopper{}'s planning engine is an augmented version of the prior IPyHOP planner \cite{bansod2022HTNReplanning}.
For planning, input is in the form of an initial task list, initial state, and domain
description.  The domain description includes tasks, primitive
actions, and method definitions.
The initial tasks are repeatedly decomposed into simpler tasks and then finally
actions based on the domain description.
The decomposition process forms a solution tree by a depth-first traversal and every intermediate
state is saved in the tree for backtracking. When a task cannot be successfully decomposed, a new decomposition
is attempted of the most recent task expanded. When every task has
been decomposed and all actions' preconditions are established,
planning has successfully completed and the actions of the tree in preorder constitute the plan.
If the planner backtracks to the sentinel root node, which is the parent of all input tasks, planning has
failed: no decomposition can achieve the task list in order.

For plan repair, \ipyhopper{} restarts the planning process at the
parent of the immediate parent of a failed action using the current state in place of the stored state.
Initially, \ipyhopper{} restricts the
process to this subtree and only backtracks further up the tree when all decompositions in the subtree fail.
Once it finds a valid decomposition, we simulate the action execution going forward. If our simulation completes, the
plan is repaired and the process is terminated. If \ipyhopper{} encounters a future simulated failure, it will redo the repair process.
This simulation-repair cycle continues until either the plan successfully repaired or root is reached, indicating that
no repaired plan is possible.



\subsection{Plan Repair by Problem Rewriting}
\label{sec:rewrite-alg}

The two methods we have discussed above both share the core pattern of
resuming the planning process after some appropriate change to the
search process.  They generate a repaired plan by redoing some portion
of planning process.  The \emph{rewrite} method of \hetal{}~\cite{HollerHTNPlanRepair2020} is very
different: it operates by generating a new problem and domain
definition that is solvable iff the plan can be repaired.  These
definitions are generated by combining the original problem and domain
definitions, the original solution (plan), the position reached in
execution, and the disturbance.  They do not provide a method for
determining whether a plan repair is actually required, so a repair
problem must be solved after every disturbance.  A key advantage of
their algorithm is that it is not specific to any particular HTN
planner: any planner that accepts their input format will work.

The central intuition behind the problem/domain method is to force the
planner to build a new plan that has as a prefix the set of actions
that were executed before the disturbance.  The final action in this
prefix is modified so that its effects include the disturbance
effects.  Any decomposition plan that is consistent with the observed
actions and that contains an executable suffix that performs all the
initial tasks, and achieves any specified goals.\footnote{Their HDDL~\cite{Hoeller20HDDL}
  input notation permits problems that have both initial task networks
\emph{and} goals.}
This definition accounts for the distinction between repairs permitted
by rewrite and those of \shopfixer{} and \ipyhopper{}. The latter
systems accept repaired plans that include methods that have been
\emph{abandoned} and their tasks achieved through new decompositions
not consistent with the original plan: rewrite does not.

\paragraph{Rewrite algorithm implementation}

No runnable implementation of \hetal{}'s
algorithm was available,\footnote{Daniel H\"oller, personal
  communication, 26 September 2023.} so we implemented it ourselves; we will share our
implementation on GitHub under an open source license.  Our
implementation follows the original definition in using HDDL for its
input and output formats.  Our implementation \emph{differs} from the
original definition in being able to handle action and method
\emph{schemas}, rather than only handling ground actions and methods
(\ie, it is a \emph{lifted} implementation).
This required extensions to some parts of the original algorithm.

\rewrite{} generates a new planning domain and
problem, so in theory it may be coupled with any HTN planner. In
practice, since HTN problem definitions are less
standardized than classical ones, there are limits to this
flexibility.  Our implementation returns a lifted plan repair problem that can be
used directly by the lifted HTN planner SHOP3~\shop{}
\cite{GoldmanKuter:SHOP3ELS}, and that can be grounded for use with
grounded planners.

We had originally intended to report on experiments that used both
\shop{} and
Panda \cite{HoellerETAL:PANDAFramework:2021} as planners for the repair
problems.  Unfortunately, we
found that Panda was unable to handle the benchmark domains we have
used in our experiments, namely, Rovers, Satellite, and OpenStacks as
reported next section.  These domains all use the ADL dialect of
PDDL/HDDL, featuring quantified goals and conditional effects.
The parsing and grounding methods used in Panda were not
able to handle the demands of ADL domains (we confirmed this with
Panda developers), so we had to limit ourselves to using only
\shop{}.\footnote{None of the satellite problems could be parsed by
  Panda in 5 minutes, only 7 of the rovers, and 9
  of the openstacks.  The 7 rovers problems could be
  grounded, but only 7 of the 9 openstacks problems.  Details
  available upon request.}
We refer to this combination as \rsthree{}.
However, since \shop{} and Panda would be solving the
same problems, we are still testing the essential features of the
rewrite algorithm.

%

\paragraph{Summary}

The \rewrite{} algorithm is most appropriate for problems where the
structure of the plan tree is critical to correctness (e.g., the toll
example, where movements and payments must be balanced by the tree),
but it may fail where disturbances put the agent into a dead end that
it will have to ``back out" of.
\ipyhopper{}
and \shopfixer{}
will be the opposite: both allow for deviations in the plan tree, so
both will easily handle cases that involve backing up to reverse a
deviation and then resuming.
They differ in that
\ipyhopper{} will more efficiently handle deviations with immediate
impact, and \shopfixer{} can better handle deviations with delayed
impact, at the expense of computation that will be wasted on simple
cases.




==> qualitative-differences.tex <==
The three algorithms analyzed in this paper have important qualitative
differences that color the experimental results and are critical to
their interpretation. (1) \rewrite{}'s definition of plan repair is more stringent
than the others; we have found benchmark planning problems that
\ipyhopper{} and/or \shopfixer{} solve but that \rewrite{} considers
unsolvable.
There are two substantial differences between \shopfixer{} and \ipyhopper{}:
(2) \shopfixer{} attempts to detect when a plan \emph{will be} invalid, before
any actions actually fail; it invests in data
structures and computation in order to detect problems as
soon as possible. \ipyhopper{}'s projections are not
model-based: it relies on an
external simulation to do projection for it, instead of having an
internal action model as most planners do.
(3) \shopfixer uses backjumping to more efficiently find repairs,
whereas \ipyhopper{} uses simple chronological backtracking. Once
again, this involves more complexity in \shopfixer{}, both in the
algorithm and in its run-time data structures.
These differences lead to different plan repair behaviors.

These differences are not simply a matter of one repair method being
``better'' than another: instead, different repair methods are
better in different situations.
The more stringent definition offered by \rewrite{} is
better when an HTN method library captures important
considerations about what sequences of actions are and are not correct
plans; the more relaxed definition better when the precise
trajectory is less important.  \shopfixer{}'s plan repair approach is
better if the costs of wrong actions are higher than the
costs of computation, \eg{} when actions are particularly expensive,
or when deferring repair could leave the agent trapped in a
dead end.  When a situation is more forgiving and
when it changes frequently, \shopfixer{}'s aggressive repair strategy
will not be worthwhile.  In the following, we give simple examples
that illustrate these differences.

The \rewrite{} paper~\cite{HollerHTNPlanRepair2020} defines a repaired
plan as one that, among other considerations, has a plan
(decomposition) tree that is a refinement of the plan tree of the
initial plan. This definition can exclude some repairs that seem
intuitively plausible.

Consider an HTN plan domain for inter-city
travel that has two alternative methods: rail and air travel.  For rail travel, we take the bus to the station, embark, travel, and
then debark. Similarly, to fly we take the bus to the airport, get on
the plane, fly, and then deplane.  Each method has the precondition
that the train station (resp., airport) be open.  Starting from home,
Panda \cite{HoellerETAL:PANDAFramework:2021} and \shop{} \cite{GoldmanKuter:SHOP3ELS} both
can find plans for air and rail travel.

Consider the plan repair problem that occurs when we take the bus to
the train station and discover that the train station is closed.
\shopfixer{} and \ipyhopper{} will detect the problem, identify
that the original \texttt{rail-travel} method cannot be fixed, and switch to air travel. However, \rewrite{} cannot repair this plan, because
the resulting plan -- bus to train station, bus to airport, embark,
fly, deplane -- is ill-formed: no expansion of the
top level goal contains \emph{both} ``bus to train station'' \emph{and} ``bus
to airport.''

This highlights a tradeoff between flexibility and efficiency that the authors of HTN domain descriptions typically face. If the HTNs use strong search-control strategies 
and knowledge to make planning efficient by quickly finding a good and acceptable solution, then those HTNs are usually not flexible enough to allow exploring alternative plans for in hierarchical plan repair. As the above example shows, the \rewrite\ algorithm commits to the 
prefix of the hierarchy for planning reasons, but that excludes possible repairs at the higher
levels of the hierarchy when a discrepancy occurs. \shopfixer and \ipyhopper are similar in that
limitation for general cases but they provide backtracking and backjumping strategies that can alleviate this limitation in some classes of domains. Section \ref{sec:results} discuss examples  of this phenomenon in our experimental results.


The \rewrite paper gives an example that shows
the rationale for its more restrictive definition of
plan repair.  In this example, the agent drives through a city
that has congestion pricing, and must pay a toll for each road segment
driven in the congestion zone.  Solution plans have the form
$x^{*} a^n b^n x^{*}$: there are actions before and after travel
in the congestion zone (the two $x^{*}$'s), then $n$
segments traveled in the congestion zone ($a^n$), followed by $n$ toll
payments ($b^n$).  The structure of the HTN methods is the mechanism
that enforces the $a^{n}$-$b^n$ balance, so if extraneous actions were
allowed, incorrect (unbalanced) plans could be derived.

\shopfixer{} and \ipyhopper{} share the same model of plan repair,
which holds that any HTN method may be re-done -- \ie, its plan
regenerated and then executed from the method's beginning, as long as
the method's preconditions hold in the state in which it begins.  As we
have seen above, that means that the ``intercity-travel'' task may be
restarted after the agent has reached the train station and discovered
that it is closed.  The difference between the two is how they attempt
to detect future action failures.

When building a repairable plan, \shopfixer{} creates a
decomposition tree that records task decompositions into subtasks, with cross-links from actions that establish facts to the actions and methods whose preconditions consume those facts.  This trades some pre-computation and storage for more rapid
detection of possible plan failures -- and detection of cases where
unexpected effects do not cause plan failures.  An example
\shopfixer{} tree is shown in Figure~\ref{fig:SHOPplan}.
%


\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{plan-tree}
  \caption{\shop{} plan tree for a rover plan; decomposition edges are
    in black; dependency cross-edges in dashed blue. Edges from the
    diamond node represent dependencies on initial state facts.}
  \label{fig:SHOPplan}
\end{figure}

\ipyhopper{}, in contrast, does not precompute any data
structures for identifying plan failures.  Instead, when
notified of a plan disturbance, it simulates the existing plan forward
in time to find impending failures.  When it finds such a failure, it
unexpands the simulated action's parent node in the solution
tree, and attempts to find a new decomposition for that
node that will not fail.  If no such decomposition exists, the parent's parent is similarly
unexpanded; this continues up the solution tree until either a valid decomposition is found
or the root is reached, which means no repair exists. 


If a valid decomposition is found, \ipyhopper{} restarts the simulation at the leftmost action of the decomposition
in postorder traversal.  This continues until either the plan
completes successfully or another failure is simulated.  If another
failure is simulated, the repair process is repeated and eventually either
the simulation will complete and the plan is repaired or the root will
be reached and repair has failed. 





==> replication.tex <==

\paragraph{Data and Code Availability.}

Upon acceptance, all materials for replication will be made
publicly available.


\label{sec:replication}
\label{sec:data-and-code}


